Dynamics and stability of U(1) spin liquids beyond mean-field theory: Triangular-lattice $J_1$-$J_2$ Heisenberg model

Quantum spin liquids (QSLs) are long-range entangled phases of frustrated magnets exhibiting fractionalised spin excitations. In two dimensions, there is limited analytical understanding of their excitation spectra beyond parton mean-field theories, which fail to capture many features of the finite frequency dynamical response. We use a self-consistent mean-field theory combined with the random phase approximation (RPA) for the $J_1$-$J_2$ Heisenberg model on the triangular lattice to describe the strong spinon-spinon interactions of the U(1) Dirac QSL. We obtain quantitative results for the dynamical spin structure factor and phase diagram compatible with comprehensive numerical efforts. We show the continuum response at the Brillouin zone corners is described by a spinon-exciton hybridised with monopole gauge excitations. We further show that the transition from the QSL to 120-degree coplanar order is in the QED$_3$ O(3)-GN universality class. We extend the method to chiral QSLs and XXZ anisotropy, and discuss its broad range of applicability to other models and for describing inelastic neutron scattering experiments in KYbSe$_2$.

==> feynmf/Makefile <==
# Makefile -- install feynmf.
# Copyright (C) 1994,1995 Thorsten.Ohl@Physik.TH-Darmstadt.de
#
# Feynmf is free software; you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by 
# the Free Software Foundation; either version 2, or (at your option)
# any later version.
#
# Feynmf is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the 
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program; if not, write to the Free Software
# Foundation, Inc., 675 Mass Ave, Cambridge, MA 02139, USA.
#
# $Id: Makefile,v 1.27 1996/12/02 09:20:35 ohl Exp $
#
########################################################################

VERSION = 1
RELEASE = 08
STATUS  = 

########################################################################

# Directories
prefix = $(HOME)
bindir = $(prefix)/bin
mandir = $(prefix)/man/man1
texdir = $(prefix)/tex/inputs
mfdir = $(prefix)/mf/inputs
docdir = $(texdir)/doc

# Commands
INSTALL = install -c -m 755
INSTALL_DATA = install -c -m 644
# INSTALL = cp
# INSTALL_DATA = cp

# This has to be the new LaTeX
LATEX = latex
# This should be the old LaTeX
LATEX209 = tex '&latex209'
# This must not have the cmbase preloaded:
MF = mf
MP = mp
MAKEINDEX = makeindex

# Your local printer mode
MFMODE = laserjet

########################################################################
# No user serviceable parts below:
########################################################################

RESOLVE_XREF = \
  $(LATEX) $*.drv && \
  while grep 'Rerun to get cross-references right\.' $*.log; \
  do \
    $(LATEX) $*.drv; \
  done

RESOLVE_XREF209 = \
  $(LATEX209) $*.drv && \
  while grep 'Rerun to get cross-references right\.' $*.log; \
  do \
    $(LATEX209) $*.drv; \
  done

RUN_METAFONT = \
  $(MF) '\mode:=$(MFMODE); input fmfsamp1'; \
  $(MF) '\mode:=$(MFMODE); input fmfsamp2'; \
  $(MF) '\mode:=$(MFMODE); input fmfsamp3'; \
  $(MF) '\mode:=$(MFMODE); input fmfsamp4'

RUN_METAPOST = \
  $(MP) fmfsamp1; \
  $(MP) fmfsamp2; \
  $(MP) fmfsamp3; \
  $(MP) fmfsamp4;

RUN_MAKEINDEX = \
  $(MAKEINDEX) -s gind.ist -o $*.ind $*.idx && \
  $(MAKEINDEX) -s gglo.ist -o $*.gls $*.glo

MANPICS = manpics.1 manpics.2 manpics.3

all: feynmf.sty feynmf.mf feynmf.drv \
     feynmp.sty feynmp.mp feynmp.drv $(MANPICS) \
     feynmf.1

all209: feynmf209.sty feynmf.mf feynmf209.drv \
	feynmp209.sty feynmp.mp feynmp209.drv $(MANPICS)

man: fmfman.dvi

man209: fmfman209.dvi

quick-man:
	$(MAKE) man RUN_MAKEINDEX=: RESOLVE_XREF=:

dvi: feynmf.dvi

dvi209: feynmf209.dvi

quick-dvi:
	$(MAKE) dvi RUN_MAKEINDEX=: RESOLVE_XREF=:

bigtest: feynmf.dvi feynmp.dvi fmfman.dvi fmfmanps.dvi manual.ps

bigtest209: feynmf209.dvi feynmp209.dvi fmfman209.dvi \
	    fmfman209ps.dvi manual209.ps

install: all
	$(INSTALL_DATA) feynmf.mf $(mfdir)
	$(INSTALL_DATA) feynmp.mp $(mfdir)
	$(INSTALL_DATA) feynmf.sty $(texdir)
	$(INSTALL_DATA) feynmp.sty $(texdir)
	$(INSTALL_DATA) feynmf.1 $(mandir)
	$(INSTALL) feynmf.pl $(bindir)/feynmf

install.doc: all
	$(INSTALL_DATA) feynmf.dtx $(docdir)
	$(INSTALL_DATA) feynmf.drv $(docdir)
	$(INSTALL_DATA) fmfman.drv $(docdir)
	$(INSTALL_DATA) $(MANPICS)  $(docdir)

uninstall:
	rm -f $(mfdir)/feynmf.mf
	rm -f $(mfdir)/feynmp.mp
	rm -f $(texdir)/feynmf.sty
	rm -f $(texdir)/feynmp.sty
	rm -f $(bindir)/feynmf
	rm -f $(mandir)/feynmf.1

uninstall.doc:
	rm -f $(docdir)/feynmf.dtx
	rm -f $(docdir)/feynmf.drv
	rm -f $(docdir)/fmfman.drv

feynmf.sty: feynmf.dtx feynmf.ins
	$(LATEX) feynmf.ins

feynmf209.sty: feynmf.dtx feynmf209.ins
	$(LATEX209) feynmf209.ins

feynmf.mf feynmf.drv feynmp.sty feynmp.mp feynmp.drv \
  fmfman.drv fmfmanps.drv: feynmf.sty

feynmf209.drv feynmp209.sty feynmp209.drv \
  fmfman209.drv fmfman209ps.drv: feynmf209.sty

feynmf.dvi: feynmf.dtx feynmf.drv feynmf.sty feynmf.mf $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAFONT)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

feynmf209.dvi: feynmf.dtx feynmf209.drv feynmf209.sty feynmf.mf $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAFONT)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

feynmp.dvi: feynmf.dtx feynmp.drv feynmp.sty feynmp.mp $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAPOST)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

feynmp209.dvi: feynmf.dtx feynmp209.drv feynmp209.sty feynmp.mp $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAPOST)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

fmfman.dvi: feynmf.dtx fmfman.drv feynmf.sty feynmf.mf $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAFONT)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

fmfman209.dvi: feynmf.dtx fmfman209.drv feynmf209.sty feynmf.mf $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAFONT)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

fmfmanps.dvi: feynmf.dtx fmfmanps.drv feynmp.sty feynmp.mp $(MANPICS)
	-$(LATEX) $*.drv
	$(RUN_METAPOST)
	-$(LATEX) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF)

fmfman209ps.dvi: feynmf.dtx fmfman209ps.drv feynmp209.sty feynmp.mp $(MANPICS)
	-$(LATEX209) $*.drv
	$(RUN_METAPOST)
	-$(LATEX209) $*.drv
	$(RUN_MAKEINDEX)
	$(RESOLVE_XREF209)

manual.ps.gz: manual.ps
	gzip < $< > $@

manual.ps: fmfmanps.dvi $(MANPICS)
	dvips -o $@ $<

manual209.ps: fmfman209ps.dvi $(MANPICS)
	dvips -o $@ $<

manpics.1: manpics.mp
	-mp $<

manpics.2 manpics.3: manpics.1

feynmf.1: feynmf.pl
	pod2man --section 1 \
	        --release "FeynMF Version $(VERSION).$(RELEASE)$(STATUS)" \
	        --center "Contributed LaTeX Utilities" $< > $@

clean:
	rm -f fmfsamp?.* \
	      *.tfm *.*gf *.*pk \
	      *.log *.t[1-9] *.t[1-9][0-9] *.t[12][0-9][0-9] \
	      *.dvi *.aux *.toc *.ilg *.glo *.gls *.idx *.ind \
	      *.ps *.mpx '#*#' *~ .*~

realclean: clean
	rm -f feynmf.mf feynmf.sty feynmf.drv feynmp.* fmfman* \
	      feynmf209.sty feynmf209.drv feynmp209.*

distclean: realclean

########################################################################
# Maintenance:

DISTFILES = /usr/local/etc/COPYING README Makefile feynmf.dtx \
	    feynmf.ins feynmf209.ins manpics.mp $(MANPICS) \
	    feynmf.pl template.tex

distdir = feynmf-$(VERSION).$(RELEASE)$(STATUS)
CVSTAG = FEYNMF_$(VERSION)_$(RELEASE)$(STATUS)
TEXTAG = v$(VERSION).$(RELEASE)
M = 

fileversion:
	perl -pe \
	  's/^\\def\\fileversion\{.*\}/\\def\\fileversion{$(TEXTAG)}/;' \
	  feynmf.dtx > feynmf.vtmp
	if cmp -s feynmf.dtx feynmf.vtmp; then \
	  rm -f feynmf.vtmp; \
	else \
	  mv feynmf.vtmp feynmf.dtx; \
	fi
	
commit: fileversion
	@if test -n "$(M)"; then \
	  echo "cvs commit -m '$(M)'"; cvs commit -m '$(M)'; \
	  echo "cvs tag $(CVSTAG)"; cvs tag $(CVSTAG); \
	  echo "cvs tag -b $(CVSTAG)_"; cvs tag -b $(CVSTAG)_; \
	else \
	  echo "usage: make commit M='<message>'" 1>&2; \
	fi

dist: $(distdir).tar.gz
snap: feynmf-current.tar.gz

$(distdir).tar.gz:
	rm -fr $(distdir) $(distdir).tmp
	cvs export -r $(CVSTAG) -d $(distdir).tmp feynmf
	mkdir $(distdir)
	(cd ./$(distdir).tmp && \
         make $(DISTFILES) && \
         cp $(DISTFILES) ../$(distdir))
	tar cf - $(distdir) | gzip > $@
	rm -fr $(distdir) $(distdir).tmp

feynmf-current.tar.gz: $(DISTFILES) fileversion
	rm -fr feynmf-current
	mkdir feynmf-current
	touch feynmf-current/1_THIS_IS_A_SNAPSHOT_OF_
	touch feynmf-current/2_WORK_IN_PROGRESS_AND__
	touch feynmf-current/3_NOT_YET_RELEASED_CODE_
	cp $(DISTFILES) feynmf-current
#	perl -pe \
#	  's/\[\\filedate/[(UNRELEASED and UNSUPPORTED snapshot)/;' \
	  feynmf.dtx > feynmf-current/feynmf.dtx
	tar cf - feynmf-current | gzip > $@
	rm -fr feynmf-current

########################################################################
# Local Variables:
# mode:text
# End:


==> feynmf/README <==
# $Id: README,v 1.30 1996/12/02 01:38:45 ohl Exp $
########################################################################

    This is feynmf, a combined LaTeX/Metafont package for easy drawing
    of professional quality Feynman diagrams.  feynmf lays out most
    diagrams satisfactorily from the structure of the graph without
    any need for manual intervention.  Nevertheless all the power of
    Metafont is available for more obscure cases.  See the
    documentation for appetizers, examples and more details.

    A preformatted manual (`manual.ps.gz') is provided to wet your
    appetite with numerous examples.

    Anyway, you are invited to share, use, abuse, and improve it, see
    the file COPYING for details.

    Enjoy,
    -Thorsten

########################################################################

   Installation:

   You need a recent LaTeX (LaTeX2e, as of December 1994 is
   sufficient) to use feynmf,  docstrip.tex to install it and doc.sty
   to typeset the documentation.  If it is not already on your system,
   you can get all this (and much more) from your nearest CTAN host.

   To install, either use the Makefile or use the installation file
   feynmf.ins:

     $ latex feynmf.ins

   then you can typeset the documentation by

     $ latex fmfman.drv
     $ mf '\mode:=laserjet; input fmfsamp1'
     $ mf '\mode:=laserjet; input fmfsamp2'
     $ mf '\mode:=laserjet; input fmfsamp3'
     $ mf '\mode:=laserjet; input fmfsamp4'
     $ latex fmfman.drv
     $ makeindex -s gind.ist -o fmfman.ind fmfman.idx
     $ makeindex -s gglo.ist -o fmfman.gls fmfman.glo
     $ latex fmfman.drv

   or by using the Makefile (`make man').  That's it.

   There is also a simple example `template.tex' that you can use as
   a template for your own creations.  To typeset, either use the
   feynmf script

     $ feynmf template

   or run Metafont manually

     $ latex template
     $ mf '\mode:=localfont; input fmftempl'
     $ latex template

   Finally, there is another installation file for LaTeX 2.09 compatible
   versions: feynmf209.ins.  This file has to be processed _in addition_
   to feynmf.ins!

########################################################################

WARNING:

    If LaTeX fails with `Unknown graphics extension: 3', you have a
    slightly out-of-date graphics.sty file (LaTeX will have issued a
    warning in this case).  There has been a change to the user
    interface, which makes it very hard to support both versions.
    Sorry.  I have chosen to support the current one, which will
    hopefully be stable.

    You can work around this by either getting a more recent graphics
    package from CTAN (macros/latex/packages/graphics) or by using
    epsf.sty instead (`\let\includegraphics\epsffile\input epsf.sty').
    [You can also ignore it and get the preformatted manual.  But you
    will not be able to use the MetaPost version in this case.]

########################################################################

    Comments, bug reports and improvements are welcome at:

        Thorsten.Ohl@Physik.TH-Darmstadt.de
        (aka: ohl@crunch.ikp.physik.th-darmstadt.de)

    New versions can be found in:

        crunch.ikp.physik.th-darmstadt.de:/pub/ohl/feynmf

    or at CTAN:

        {ftp.shsu.edu,ftp.tex.ac.uk,ftp.dante.de}:
          ... macros/latex/contrib/supported/feynmf

    There are two mailing lists

        feynmf-announce@crunch.ikp.physik.th-darmstadt.de
        feynmf-bugs@crunch.ikp.physik.th-darmstadt.de

    both are open for subscription.  The former should be very low
    volume and carry only important announcements.  The latter can
    serve as a more general discussion forum.

    To subscribe, send mail to

        majordomo@crunch.ikp.physik.th-darmstadt.de

    and NOT to the lists itself.  The following commands (on a line in
    the body of the mail, not in the subject) are useful: `subscribe
    feynmf-announce', `unsubscribe feynmf-bugs', `help', etc.

########################################################################

NEWS for Version 1.08

    *  Improved very short gluon and photon propagators by relaxing
    overly aggressive rounding.

    *  New (still experimental) `feynmf' script automating the
    invocation of Metafont (requires perl(1)).

NEWS for Version 1.07

    *  Switch off I/O during the first pass in AMS-LaTeX equation
    environments.  This avoids a nasty race condition (thanks to Axel
    Thimm for reporting this bug).  A beneficial side effect is that
    it saves us 50% processing time in these cases.

NEWS for Version 1.06

    *  New abstraction: polygons.  Useful for complex vertices in
    non-perturbative diagrams.

    *  New commands: \fmfpoly, \fmfpolyn and \fmfrpolyn, implementing
    polygons.

    *  New option `rubout' for crossing propagators.

    *  Some common typos are detected are appropriate warning messages
    are issued.

    *  New options `errorstop', `scroll', `nonstop' and `batch' for
    specifying the desired interactionmode.

    *  Work around an obscure babel/german/feynmf three way
    destructive interference.

NEWS for Version 1.05

    *  FeynMF now coexists with french.sty and other packages that
    change the \catcode of ``:''.

    *  Fixed a bug introduced in version 1.03, which could cause
    problems with font loading.  Unfortunately, the fix has to give up
    some compatibility with earlier versions.  Sources for version
    1.02 and earlier which used \noexpand in labels have to upgraded
    or the option `pre-1.03' has to be used.  Sorry.

NEWS for Version 1.04

    *  Finally, \fmffixed{(dx,whatever)}{v1,v2} and
    \fmffixed{(whatever,dy)}{v1,v2} do what you would expect them
    to.  \fmffixedx and \fmffixedy are new synonyms for those.

NEWS for Version 1.03

    *  It is no longer necessary to protect TeX command sequences with
    \noexpand.  Old files using \noexpand will continue to work.

NEWS for Version 1.02

    *  Read the .tfm file before writing the .mf file destructively.
    This should allow a transparent two pass processing if MakeTeXTFM
    is enabled.  Thanks to Thomas Esser <te@informatik.uni-hannover.de> 
    for the suggestion.

NEWS for Version 1.01

    * new decoration shapes for vertices by popular demand: `cross'
    (also `triacross', `pentacross' and `hexacross').

    * fixed a rounding bug in cut-off ends (noticeable as a spurious
    thin diagonal line at the left end of double lines).

    * The maximum size for shaded and hatched areas has been doubled
    by removing an obsolete speedup hack that was not used anymore.

    * In an unrelated move, shading and hatching has been
    reimplemented in a much more general fashion.  Now arbitray
    tilings can be specified as argument to `decoration.filled='.  The
    old style numerical arguments continue to work, but should be
    replaced by `empty', `full', `shaded', and `hatched' in new
    documents.

########################################################################
# Local Variables:
# mode:indented-text
# End:

